Tunable Electronic Properties and Large Rashba Splittings Found in Few-Layer Bi$_2$Se$_3$/PtSe$_2$ Van der Waals Heterostructures

We use first-principles calculations to show that van der Waals (vdW) heterostructures consisting of few-layer Bi$_2$Se$_3$ and PtSe$_2$ exhibit electronic and spintronics properties that can be tuned by varying the constituent layers. Type-II band alignment with layer-tunable band gaps and type-III band alignment with spin-splittings have been found. Most noticeably, we reveal the coexistence of Rashba-type spin-splittings (with large $\alpha_{\rm R}$ parameters) in both the conduction and valence band stemming from few-layer Bi$_2$Se$_3$ and PtSe$_2$, respectively, which has been confirmed by spin-texture plots. We discuss the role of inversion symmetry breaking, changes in orbital hybridization and spin-orbit coupling in altering electronic dispersion near the Fermi level. Since low-temperature growth mechanisms are available for both materials, we believe that few-layer Bi$_2$Se$_3$/PtSe$_2$ vdW heterostructures are feasible to realize experimentally, offering great potential for electronic and spintronics applications.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
